Exploring Transformer's potential on automatic piano transcription

Most recent research about automatic music transcription (AMT) uses convolutional neural networks and recurrent neural networks to model the mapping from music signals to symbolic notation. Based on a high-resolution piano transcription system, we explore the possibility of incorporating another powerful sequence transformation tool -- the Transformer -- to deal with the AMT problem. We argue that the properties of the Transformer make it more suitable for certain AMT subtasks. We confirm the Transformer's superiority on the velocity detection task by experiments on the MAESTRO dataset and a cross-dataset evaluation on the MAPS dataset. We observe a performance improvement on both frame-level and note-level metrics after introducing the Transformer network.

==> tables/tb_res_pos.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[thb!]
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
 & \textbf{MAE} & \textbf{STD} \\ \midrule
With positional encoding & \textbf{4.0026} & \textbf{4.0077} \\
Without positional   encoding & 4.4241 & 4.3072 \\ \bottomrule
\end{tabular}
\caption{Comparison of CNN-Transformer with or without positional encoding. MAE and STD refer to the mean and standard deviation of velocity prediction's absolute error, respectively.}
\label{tab:res-pos}
\end{table}
